Time-Shared Execution of Realtime Computer Vision Pipelines by Dynamic Partial Reconfiguration

This paper presents an FPGA runtime framework that demonstrates the feasibility of using dynamic partial reconfiguration (DPR) for time-sharing an FPGA by multiple realtime computer vision pipelines. The presented time-sharing runtime framework manages an FPGA fabric that can be round-robin time-shared by different pipelines at the time scale of individual frames. In this new use-case, the challenge is to achieve useful performance despite high reconfiguration time. The paper describes the basic runtime support as well as four optimizations necessary to achieve realtime performance given the limitations of DPR on today's FPGAs. The paper provides a characterization of a working runtime framework prototype on a Xilinx ZC706 development board. The paper also reports the performance of realtime computer vision pipelines when time-shared.

==> 9_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Even as FPGAs are increasingly used in computing, they are
nevertheless deployed more often like ASICs. With DPR, FPGAs
hold the promise of becoming a more dynamic and flexible shared
resource in computing use.  In this paper, we presented our
investigation to apply DPR at the time scale of individual
frames to time-share an FPGA by multiple realtime vision pipelines.

 Nevertheless, the
current runtime framework is restrictive due to the high
reconfiguration time. 








%FPGAs, especially DPR, is still a very much under tapped capability
%in casting FPGAs as a 
%context where an FPGA's fabric is time-multiplexed by multiple
%pipelines at a frame granularity using DPR. However, challenges such
%as asynchronous module execution, rate mismatch and wasteful
%reconfigurations arise in this new mode of operation. We presented
%the theory and techniques for solving those challenges and
%implemented them in a proof-of-concept runtime framework using
%DPR. Our evaluation shows that it is possible to interleave multiple
%vision pipelines at a frame granularity. We achieve realtime
%requirements with a 2 to 3x performance degradation factor compared
%to a non-interleaved design, making this mode of operation viable
%only for non highly constrained vision systems.


%%
%%We presented the techniques for hiding and reducing
%%reconfiguration time. First, we decouple pipeline stages to overlap
%%reconfiguration and processing within a pipeline time-slice. Second,
%%the framework supports round-robin scheduling at the granularity of
%%macro frames to amortize reconfiguration cost. Third, the framework
%%can drive pipelines with downsampled camera stream in a fashion
%%transparent to the pipelines. Lastly, we designed an interconnect
%%infrastructure to reduce the number of reconfigurations in scenario
%%where time-shared pipelines share common stages.  We developed a
%%runtime framework and built a vision system on top of it to evaluate
%%the effectiveness of our techniques. Through an application-level
%%performance study, we showed that we managed to achieve useful frame
%%rates despite considerably high reconfiguration time.




